A Deep Learning Approach to Anomaly Sequence Detection for High-Resolution Monitoring of Power Systems

A deep learning approach is proposed to detect data and system anomalies using high-resolution continuous point-on-wave (CPOW) or phasor measurements. Both the anomaly and anomaly-free measurement models are assumed to have unknown temporal dependencies and probability distributions. Historical training samples are assumed for the anomaly-free model, while no training samples are available for the anomaly measurements. By transforming the anomaly-free observations into uniform independent and identically distributed sequences via a generative adversarial network, the proposed approach deploys a uniformity test for anomaly detection at the sensor level. A distributed detection scheme that combines sensor level detections at the control center is also proposed that combines local detections to form more reliable detections. Numerical results demonstrate significant improvement over the state-of-the-art solutions for various bad-data cases using real and synthetic CPOW and PMU data sets.

==> viewgr.tex <==
%
%  vgmac.tex -- viewgraph macros for tex
%
%               vgmac is intended for use with the 12pt article style.
%               The commands currently suported are:
%               
%               Format commands:
%                  \horizfmt - horizontally formatted vg's
%                  \vertfmt  - vertically     "       "     (default)
%
%               Fonts:
%                  \bodyfont - std. font for body of vg     (default)
%                  \bodysmall - small font for body of vg
%                  \bodybold -  bold   "    "   "   "   "
%                  \bodyital - italic  "    "   "   "   "
%                  \titlefont - large font used for vg titles
%
%               Pagestyles:
%                  vgdatelabel - footer with left-justified filename
%                                and runtime, right-justified
%                                pagenumber                 (default)
%                  vgemptydatelabel - footer with left-justified runtime
%                                     and right-justified file name
%
%                 *N.B. if the filenames are relative to the current
%                       directory, the true path will appear in the footer
%                       only if the user has the following alias for latex:
%
%                       alias latex 'latex \\def\\dirname\{`pwd`\}\\input '
%
%               Page Initialization:
%                  \invg#1 - command to input a new viewgraph file.
%                            vg files are each assumed to contain a
%                            single vg.  #1 is as for the \input command.
%                  \newvgtitle#1 - command to initialize a vg with
%                                  title #1
%                  \newvgempty   - command to initialize a vg with no title
%
%                 *N.B. The first command in each vg file must be
%                       either \newvgtitle or \newvgempty
%
%               Text Layout:
%                  \leftitem#1 -      a bulleted, hanging indentation,
%                                     raggedright paragraph with contents #1
%                  \indentedpar#1#2 - a centered narrow paragraph #2
%                                     with bold label #1
%                  \bigskip -         has been redefined with infinite stretch
%
%                 *N.B. It is recommended that items in the viewgraph
%                       be seperated with \bigskip's
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  $Header: /user2/marcg/tex/macros/RCS/vgmac.tex,v 1.3 1992/02/11 01:20:42 marcg Exp marcg $
%
%  $Log: vgmac.tex,v $
%  Revision 1.3  1992/02/11  01:20:42  marcg
%  added \bodytiny and \bodytinyital
%
%  Revision 1.2  1991/03/19  01:10:40  marcg
%  added \par to \indentedpar
%
%  Revision 1.1  91/02/22  10:10:13  marcg
%  Initial revision
%  
%               
%  marcg, 1/22/91, Initial commented version
%  marcg, 1/29/91, Improved footer filename handling
%  marcg, 2/11/91, local definition of \xxvpt 
%  marcg, 2/20/91, changed def of indentedpar to use current value of 
%                  \textwidth
%  marcg, 2/21/91, replaced definition of \xxvpt with initialization
%                  of \@xxvpt for relative independence from
%                  lfonts.tex.  Dick mentioned that the rascals
%                  version of lfonts uses 25pt fonts in \xxvpt, while
%                  many other systems use 20pt fonts there.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\typeout{vgmac package, $Revision: 1.3 $, $Date: 1992/02/11 01:20:42 $}
%
% page layout and fonts 
%
\oddsidemargin -.25truein \topmargin -.25truein 
\headheight 0pt \headsep 0pt \topskip 0pt
\renewcommand\baselinestretch{1.1}
\def\magstepsix{2985}
\def\magstepseven{3583}
\font\titlefont = cmssbx10 scaled\magstep5
\font\bodyfont = cmss10 scaled\magstep4
\font\bodysmall = cmss10 scaled\magstep3
\font\bodytiny = cmss10 scaled\magstep2
\font\bodytinyital = cmssi10 scaled\magstep2
\font\bodybold = cmssbx10 scaled\magstep4
\font\bodyital = cmssi10 scaled\magstep4
\leftmargini .75 truein \rightmargin .5 truein
\leftmarginii .75 truein 
\leftmarginiii .75 truein
\leftmarginiv .75 truein
\itemsep 15pt plus 20pt minus 5pt
\def\bigskip{\vskip .9em plus 1fil minus .15em}
%
%  format comands
%
\def\horizfmt{\textwidth 9.50truein \textheight 7.0truein
\special{landscape}} 
%\special{header=/user/young/tex/macros/YMCAlandscapevglogo.ps}
\def\vertfmt{\textwidth 7.0truein \textheight 9.50truein}
%\special{header=/user/young/tex/macros/YMCAvglogo.ps} 
%
%  \newvgtitle starts a new titled viewgraph
%  \newvgempty starts a new untitled viewgraph
%
\def\newvgtitle#1{\begin{center} \Huge\titlefont #1 \\[-.2em]
\rule{\textwidth}{2pt}
\end{center}
\LARGE\bodyfont
\raggedright
\parindent 0pt
}
\def\newvgempty{\LARGE\bodyfont\raggedright\parindent 0pt}
%
%  \invg inputs a viewgraph file and sets up footer filename as
%  follows:
%     filename starting with '/' --> footer contains filename
%     otherwise --> footer contains filename prepended with \dirname
%                   if it exists.
%
\def\invg#1{\clearpage\def\vgfilename{#1}
  \getinit{#1}
  \gdef\vglabelname{%
    \if\initchar/\else%
      \expandafter\ifx\csname dirname\endcsname\relax%
      \else\expandafter\badBgone\dirname\relax/\fi\fi%
        \expandafter\badBgone\vgfilename\relax.tex}%
\input #1}
%
%  \getinit sets the global variable \initchar to the first token of
%  its argument.
%
\newif\ifreadone  % used by \firstchar
\def\getinit#1{\firstchar#1\relax}
\def\firstchar#1{%
  \ifreadone\relax\else \gdef\initchar{#1}\readonetrue\fi%
  \if #1\relax\readonefalse\let\next=\relax%
  \else\let\next=\firstchar\fi%
  \next%
}
%
%  \leftitem yields a left justified paragraph with a bullet
%
\def\leftitem#1{\medskip
\setbox1\hbox{$\bullet$\hskip 1em}
\leavevmode\hangindent\wd1\hangafter1{\box1 #1\par}}
%
%  \indentedpar yields an narrow centered paragraph, #2, with label #1
%  The idea is to make the lines of the parbox maximally long with
%  no hyphenation and a raggedright.  The argument of the parbox used
%  to be '\raggedright #2'
%
\newdimen\indparind\indparind 3em
\newdimen\indparwd
\long\def\indentedpar#1#2{\indparwd\textwidth\advance\indparwd by -2\indparind
  {\bodybold #1:}\hfil\break
  \null\hskip\indparind\parbox[t]{\indparwd}{%
\linepenalty 10000\hyphenpenalty 10000\rightskip 0pt plus3em{#2}}\par}
%
%  makeatletter required for badBgone, ps@vgdatelabel,
%  ps@vgemptydatelabel, xxvpt
%
\makeatletter
\def\badBgone#1{\toks0={#1}\expandafter\if\the\toks0\relax%
    \let\next=\relax\else%
    \expandafter\if\the\toks0_\_%
    \else\expandafter\if\the\toks0&\&%
    \else\expandafter\if\the\toks0$\$%
    \else\expandafter\if\the\toks0^\^{ }%
    \else\expandafter\if\the\toks0<$\m@th <$%
    \else\expandafter\if\the\toks0>$\m@th >$%
    \else\expandafter\if\the\toks0##{$\m@th\sharp$}%
    \else\expandafter\if\the\toks0\noexpand{{$\m@th\{$}%
    \else\expandafter\if\the\toks0\noexpand}{$\m@th\}$}%
    \else\expandafter\if\the\toks0\noexpand%\%%
    \else\the\toks0\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi%
    \let\next=\badBgone\fi%
    \next}%
%
%
\def\ps@vgdatelabel{\let\@mkboth\@gobbletwo
     \def\@oddhead{}
     \newdimen\mydimen \mydimen=\textwidth
     \divide\mydimen by 2
     \newcount\hours \hours=\time \divide\hours by 60
     \newcount\minutes \minutes=\hours \multiply\minutes by
                           -60 \advance\minutes by\time
     \def\@oddfoot{\hbox to\textwidth{\footnotesize\sl\today, \the\hours:%
         \ifnum\minutes<10 0\fi\the\minutes\ --- %
         \vglabelname\hfill\rm\thepage}}
     \def\@evenhead{}\let\@evenfoot\@oddfoot%
     }
%
%
\def\ps@vgemptydatelabel{\let\@mkboth\@gobbletwo
     \def\@oddhead{}
     \newdimen\mydimen \mydimen=\textwidth
     \divide\mydimen by 2
     \newcount\hours \hours=\time \divide\hours by 60
     \newcount\minutes \minutes=\hours \multiply\minutes by
                           -60 \advance\minutes by\time
     \def\@oddfoot{\hbox to\mydimen{\footnotesize\sl\today, \the\hours:%
         \ifnum\minutes<10 0\fi\the\minutes\hfill}\hss%
         \hbox to\mydimen{\quad\footnotesize\sl\hfill%
         \vglabelname\hss}}
     \def\@evenhead{}\let\@evenfoot\@oddfoot%
     }
%
%  xxvpt is called by \Huge at 12pt in article style, so we initialize
%  @xxvpt to load in sanserif fonts.  This allows us to override the 
%  definition in xxvpt independent of the machine type.  This whole
%  exercise is to fix some of my math macros that use \sf
%
%\@getfont\psf\sffam\@xxvpt{\@mss\@magscale5}\normalsize
\makeatother
%
%  default is vertical format and vgdatelabel pagestyle
%
\vertfmt
\pagestyle{vgdatelabel}



